Activity Report on the Seventh African School of Fundamental Physics and Applications (ASP2022)

The African School of Fundamental Physics and Applications, also known as the African School of Physics (ASP), was initiated in 2010, as a three-week biennial event, to offer additional training in fundamental and applied physics to African students with a minimum of three-year university education. Since its inception, ASP has grown to be much more than a school. ASP has become a series of activities and events with directed ethos towards physics as an engine for development in Africa. We report on the seven African School of Physics, ASP2022, organized at Nelson Mandela University, on November~28 to December~8, 2022. ASP2022 included programs for university students, high school teachers and high school pupils.

==> expenseTable.tex <==
The total expenditures amounted to \texteuro168496 as shown in Table~\ref{tab:table2}; that left a surplus of \texteuro16835 from the DOE funds shown in Table~\ref{tab:table1}: these funds were intended to cover fourteen lecturers; however, only eleven were covered, resulting in the excess of about \texteuro17000. The surplus was earmarked towards the third African Conference of Fundamental and Applied Physics, ACP2023, planned for September 25--29, 2023, at Nelson Mandela University, George Campus, in South Africa~\cite{acp2023}.
\begin{table}[!htbp]
\centering
\begin{tabular}{l|r|r|r|r}
\hline\hline
\textbf{Item}    &  \textbf{Travel} & \textbf{Catering} &  \textbf{Lodging} & \textbf{Other}\\ \hline
ASP2022 Site Visit             &  5611 &   61  &  983   & \\ 
South African Students         &  1334 &  4473 & 3371   & \\
Local Students \& Tutors       &     0 & 17754 &      0 & \\
South African Teachers         &     0 & 17990 & 1976   & \\
South African Pupils           &     0 &  7652 &      0 & \\
Lecturers from South Africa    &   424 &       &  517   & \\ 
Local Organizers \& Lecturers  &     0 & 17082 &      0 & \\
International Students         & 29628 & 14795 &  9401  & \\
Online Participants            &       &       &        & 1541 \\
Online Networking              &       &       &        & 331 \\
International Lecturers        & 22545 &       & 5610   & \\
Local Transportation           &       &       &        & 4927 \\
Equipment \& Accessories       &       &       &        & 490 \\
\hline
Total                          & 59542 & 79807 &  21858 & 7289 \\
 \hline\hline
\end{tabular}
\caption{Expenditures for ASP2022 in Euros. Many institutes covered the travels of their staff lecturers. The table shows only travel coverage of some lecturers through DOE or NRF funds. The site visit is an important ASP event; it consists of travels of international organizers to the host country to inspect the venue and make recommendations for improvements before the school starts. For ASP2022, the site visit occurred in June 2022. }
\label{tab:table2}
\end{table}



==> supportTable.tex <==
At the time of ASP2022 preparation, the conversion rate between the Euro and the Dollar was approximately 1:1.  The summed contributions received, shown in Table~\ref{tab:table1}, amounted to \texteuro185331.
\begin{table}[!htbp]
\centering
\begin{tabular}{l|r|l}
\hline\hline
\textbf{Source}    &  \textbf{Amount} & \textbf{Currency} \\ \hline
DOE (USA)           &   56000  & Dollar     \\
NRF (South Africa) & 400000 & Rand \\
ICTP (Italy)              & 19131.06 & Euro\\
INFN (Italy)              & 15000 & Euro\\
BNL  (USA)              & 10000 & Dollar \\
University of Birmingham (UK) & 10000 & Dollar \\
Prof. Robert Lourie (USA)  & 10000 & Dollar \\
Lee Foundation (Taiwan) & 6000 & Euro \\
CERN (Switzerland) & 5000 & CHF \\
FNAL (USA)         & 5000 & Dollar \\
APS (USA) & 5000 & Dollar \\
GSSI (Italy)  & 5000 & Euro \\
DESY (Germany)  & 5000 & Euro \\
PSI (Switzerland)  & 4000 & CHF \\
Dr. Joseph Mitchell (USA) & 3500 & Dollar \\
IEEE (USA)  & 3500 & Dollar \\
 \hline\hline
\end{tabular}
\caption{Contributions to the ASP2022 budget. The DOE funds were earmarked towards coverage for fourteen lecturers from USA institutes and others who did not have travel coverage, as well as online participants.}
\label{tab:table1}
\end{table}


